Porting a sparse linear algebra math library to Intel GPUs

With the announcement that the Aurora Supercomputer will be composed of general purpose Intel CPUs complemented by discrete high performance Intel GPUs, and the deployment of the oneAPI ecosystem, Intel has committed to enter the arena of discrete high performance GPUs. A central requirement for the scientific computing community is the availability of production-ready software stacks and a glimpse of the performance they can expect to see on Intel high performance GPUs. In this paper, we present the first platform-portable open source math library supporting Intel GPUs via the DPC++ programming environment. We also benchmark some of the developed sparse linear algebra functionality on different Intel GPUs to assess the efficiency of the DPC++ programming ecosystem to translate raw performance into application performance. Aside from quantifying the efficiency within the hardware-specific roofline model, we also compare against routines providing the same functionality that ship with Intel's oneMKL vendor library.

==> sn-acks.tex <==
%\section*{Acknowledgments}

This work was supported by the ``Impuls und Vernetzungsfond'' of the Helmholtz 
Association under grant VH-NG-1241, and the US Exascale Computing Project 
(17-SC-20-SC), a collaborative effort of the U.S. Department of Energy Office 
of Science and the National Nuclear Security Administration.

The authors want to acknowledge the access to the Intel\textsuperscript{\tiny\textregistered} Devcloud early access development platform.

%The authors want to acknowledge the access to the PizDaint 
%supercomputer at the Swiss National Supercomputing Centre granted under the 
%project \#d65.


